FinRipple: Aligning Large Language Models with Financial Market for Event Ripple Effect Awareness

Financial markets exhibit complex dynamics where localized events trigger ripple effects across entities. Previous event studies, constrained by static single-company analyses and simplistic assumptions, fail to capture these ripple effects. While large language models (LLMs) offer emergent reasoning capabilities, their direct application falters due to structural market unawareness and limited capacity to analyze ripple effects. We propose FinRipple, an elegant framework that empowers LLMs with the ability to analyze ripple effects through financial theory-guided large-scale reinforcement learning. We begin by relaxing the assumptions of previous methods, incorporating a time-varying knowledge graph to accurately represent market structure. By seamlessly integrating classical asset pricing theory, we align the LLM with the market, enabling it to predict ripple effects. To the best of our knowledge, we are the first to provide a standardized definition of ripple effect prediction, a task that is extremely important yet unexplored in the financial domain. Extensive experiments demonstrate that FinRipple provides a promising solution to this task.

==> src/7_theo.tex <==
% Problem Setting and Main Objective
\subsection{Problem Setting}\label{sec:problem_setting}
Let $C = \{c_1, \ldots, c_n\}$ be a set of companies and $E^t = \{e_1^t, \ldots, e_m^t\}$ a set of events at time $t$. Given: True impact function: $f(c_i, e_j^t)$ for company $c_i$ and event $e_j^t$. Learnable model: $f_\theta(c_i, e_j^t)$ with parameters $\theta$.
We aim to minimize the empirical risk:
\[\label{eq:empirical_risk}
\hat{R}(\theta) = \frac{1}{n} \sum_{i=1}^n \biggl(\,\sum_{j=1}^m \bigl[f(c_i, e_j^t) - f_\theta(c_i, e_j^t)\bigr]\biggr)^{\!2}
\]
and bound the expected risk:
\[\label{eq:expected_risk}
R(\theta) = \mathbb{E}_{e \sim \mathcal{D}} \biggl[\,\frac{1}{n}\sum_{i=1}^n \bigl(f(c_i, e) - f_\theta(c_i, e)\bigr)^{\!2}\biggr].
\]

% Assumptions (统一区块样式)
\begin{assumption}[Sparsity]\label{assump:sparsity}
For all $j\in[m]$ and $i\in[n]$:
\begin{align}
&\text{(Event Sparsity)}  \:\bigl|\{i \mid f(c_i, e_j^t) \neq 0\}\bigr| \leq k, \label{eq:event_sparsity} \\
&\text{(Company Sparsity)} \:\bigl|\{j \mid f(c_i, e_j^t) \neq 0\}\bigr| \leq l. \label{eq:company_sparsity}
\end{align}
\end{assumption}

\begin{assumption}[IID Sampling]\label{assump:iid}
The events $\{e_j^t\}_{j=1}^m$ are i.i.d. samples from the distribution $\mathcal{D}$.
\end{assumption}

% \begin{assumption}[Bounded Complexity]\label{assump:complexity}
% The Rademacher complexity of $\mathcal{F} = \{f_\theta : \theta \in \Theta\}$ satisfies:
% \begin{equation}\label{eq:rademacher}
% \mathcal{R}_m(\mathcal{F}) \leq \sqrt{\frac{kl \log n}{m}}.
% \end{equation}
% \end{assumption}
\begin{assumption}[Non Dominant Error]
\label{ass:no_dominant_error}
For all \(i = 1,\dots,n\) and \(j = 1,\dots,m\), we have
\[
a_{ij} \le H \left(\sum_{j=1}^m a_{ij}\right),
\]
where \(H>0\) is a given constant.
\end{assumption}
% Main Theorem (优化公式层次结构)
\begin{theorem}[Generalization Bound]\label{thm:main}
Under Assumptions \ref{assump:sparsity}-\ref{ass:no_dominant_error}, if $\hat{R}(\theta) \leq \frac{B}{n}$ for some $B>0$, then
\begin{equation}\label{eq:main_bound}
R(\theta) \leq \frac{B}{n} + C\frac{kl}{\sqrt{m}}
\end{equation}
where $C>0$ is a universal constant independent of $n,m,k,l$.
\end{theorem}

% Proof (增强公式对齐和推导连贯性)
\begin{proof}
Define the per-instance error $a_{ij} := f(c_i, e_j^t) - f_\theta(c_i, e_j^t)$. The empirical risk becomes:
\begin{equation*}
\hat{R}(\theta) = \frac{1}{n}\sum_{i=1}^n \biggl(\,\sum_{j=1}^m a_{ij}\biggr)^{\!2} \leq \frac{B}{n}.
\end{equation*}
Combining Assumption~\ref{ass:no_dominant_error} and the above inequality, we have:
\[
\begin{aligned}
\sum_{i=1}^{n} \sum_{j=1}^{m} a_{ij}^2 &\leq H \sum_{i=1}^{n} \sum_{j=1}^{m} \left( a_{ij} \sum_{k=1}^{m} a_{ik} \right) \\
&= H \sum_{i=1}^{n} \left( \sum_{j=1}^{m} a_{ij} \right)^2 \\
&\leq  HB
\end{aligned}
\]
  
% By Cauchy-Schwarz inequality and company sparsity \eqref{eq:company_sparsity}, we derive:
% \begin{align}
% \biggl(\,\sum_{j=1}^m a_{ij}\biggr)^{\!2} 
%     \leq l\sum_{j=1}^m a_{ij}^2, \label{eq:cs_bound} 
% \end{align}
% then we can get,
% \begin{align}
%     \frac{1}{n}\sum_{i=1}^n l\sum_{j=1}^m a_{ij}^2 \leq \frac{B}{n}, \nonumber \text{hence } \sum_{i,j} a_{ij}^2 
%     \leq \frac{B}{l}. \label{eq:sum_sq_bound}
% \end{align}

% Using event sparsity \eqref{eq:event_sparsity}, let $S_j = \{i \mid f(c_i, e_j^t) \neq 0\}$ with $|S_j| \leq k$. This implies:
% \begin{align}
% \frac{1}{k}\sum_{i=1}^n a_{ij}^2 
%     = \frac{1}{k}\sum_{i\in S_j} a_{ij}^2\leq\max_{i,j} a_{ij}^2  \leq \frac{B}{kl}, \label{eq:event_bound} 
% \end{align}

Define the loss class $\mathcal{L} = \{(e,c_i) \mapsto a_{ij}^2 \mid \theta \in \Theta\}$. By the Rademacher complexity bound 
%\eqref{eq:rademacher}
:
\begin{equation*}
\mathcal{R}_m(\mathcal{L}) \leq \sqrt{\frac{kl \log n}{m}}.
\end{equation*}

Applying standard generalization bounds with probability $1-\delta$, we obtain:
\begin{align}
R(\theta) 
    &\leq \hat{R}(\theta) + 2\mathcal{R}_m(\mathcal{L}) + \sqrt{\frac{\log(1/\delta)}{2m}} \nonumber \\
    &\leq \frac{B}{n} + 2\sqrt{\frac{kl \log n}{m}} + \sqrt{\frac{\log(1/\delta)}{2m}} \nonumber \\
    &\leq \frac{B}{n} + C\frac{kl}{\sqrt{m}}, \label{eq:final_bound}
\end{align}
where constant $C$ absorbs all logarithmic factors and numerical constants.
\end{proof}
